AutoTune: Controller Tuning for High-Speed Flight

Due to noisy actuation and external disturbances, tuning controllers for high-speed flight is very challenging. In this paper, we ask the following questions: How sensitive are controllers to tuning when tracking high-speed maneuvers? What algorithms can we use to automatically tune them? To answer the first question, we study the relationship between parameters and performance and find out that the faster the maneuver, the more sensitive a controller becomes to its parameters. To answer the second question, we review existing methods for controller tuning and discover that prior works often perform poorly on the task of high-speed flight. Therefore, we propose AutoTune, a sampling-based tuning algorithm specifically tailored to high-speed flight. In contrast to previous work, our algorithm does not assume any prior knowledge of the drone or its optimization function and can deal with the multi-modal characteristics of the parameters' optimization space. We thoroughly evaluate AutoTune both in simulation and in the physical world. In our experiments, we outperform existing tuning algorithms by up to 90% in trajectory completion. The resulting controllers are tested in the AirSim Game of Drones competition, where we outperform the winner by up to 25% in lap-time. Finally, we show that AutoTune improves tracking error when flying a physical platform with respect to parameters tuned by a human expert.

==> sections/appendices.tex <==
\section{Supplementary}

\subsection{Tracks} \label{app:tracks}

\begin{center}
\includegraphics[width=0.49\linewidth]{images/easy.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_easy.png}
\captionof{figure}{Circle track.}
\label{fig:appendix_soccer_easy}

\includegraphics[width=0.49\linewidth]{images/drop_easy.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_drop_easy.png}
\captionof{figure}{Drop track.}
\label{fig:appendix_drop_easy}

\includegraphics[width=0.49\linewidth]{images/flip_easy.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_flip_easy.png}
\captionof{figure}{Flip track.}
\label{fig:appendix_flip_easy}

\includegraphics[width=0.49\linewidth]{images/spiral_reverse.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_spiral_reverse.png}
\captionof{figure}{Spiral track.}
\label{fig:appendix_spiral}

\includegraphics[width=0.49\linewidth]{images/qualifier.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_qualifier.png}
\captionof{figure}{Qualifier track.}
\label{fig:appendix_qualifier}

\includegraphics[width=0.49\linewidth]{images/final.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_final.png}
\captionof{figure}{Final track.}
\label{fig:appendix_final}

\includegraphics[width=0.49\linewidth]{images/rampup.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_rampup.png}
\captionof{figure}{SplitS track.}
\label{fig:appendix_real}
\end{center}

Specifically, we select the following maneuvers:
\begin{itemize}
    \item Circle: 2D maneuver with a radius of $r=\SI{16}{\meter}$. Consists of 12 waypoints at an average of \SI{9}{\meter} distance.
    \item Drop: Ascent of $\SI{21}{\meter}$ in z over $\SI{50}{\meter}$ length followed by a steep descent of $\SI{16}{\meter}$ in height. Ends with a semi-circle with radius $r=\SI{16}{\meter}$. Consists of 12 waypoints at an average of \SI{10}{\meter} distance.
    \item Flip: Ascent of $\SI{25}{\meter}$ in z over $\SI{117}{\meter}$ length, with an half-loop in z of $\SI{14}{\meter}$ radius. Ends with a steep descent of $r=\SI{20}{\meter}$ over $\SI{28}{\meter}$ length. Consists of 12 waypoints at an average of \SI{13}{\meter} distance.
    \item Spiral: Ascent of $\SI{6}{\meter}$ followed by a spiral made of three planar circles of $30$, $22$, and $16$ meters in the clockwise direction followed by a half a circle with radius $r=\SI{6}{\meter}$. Then the drone follows two planar circles of $30$ and $38$ meters in a counter-clockwise direction. Consists of 17 waypoints at an average of \SI{13}{\meter} distance.
    \item Qualifier: Track used for the qualification round of the 2019 AirSim Game of Drones competition. Made of an ascending circle of $\SI{160}{\meter}$, a $\SI{23}{\meter}$ drop in height over $\SI{25}{\meter}$ length and a long straight descent of $\SI{148}{\meter}$ length. Consists of 20 waypoints at an average of \SI{16}{\meter} distance.
    \item Final: Track used for the final round of the 2019 AirSim Game of Drones competition. Made of a $\SI{209}{\meter}$ long segment with a hairpin and loop, followed by a $\SI{40}{\meter}$ ascent over approximately $\SI{296}{\meter}$. Consists of 22 waypoints at an average of \SI{22}{\meter} distance.
\end{itemize}
%
Eventually, in the real world we fly an aggressive trajectory, that we call SplitS, composed of 21 waypoints with abrupt changes in the flight direction and speeds in the range $8-15\SI{}{\meter\per\second}$. The SplitS trajectory consists of a sequence of ascents and drops of $\SI{3}{\meter}$ in height repeated three times.
%
The trajectories of these maneuvers are illustrated in Section~\ref{app:tracks}.
%
All maneuvers start and end in the hover condition.

\subsection{Training Data and Feature Selection}

The training data consists of $14$ time-optimal trajectories, each annotated with a set of parameters that allows the controller to successfully track the trajectory.
%
In total, the training trajectories are divided into $73$ segments: $13$ flat, $22$ ascent, $23$ descent, and $15$ steep.
%
\rebuttal{For each segment type, we train a Gradient Boosting regressor on the relative data with default parameters}. We extract five features from each segment, namely the number of points in the segment, the slope of the line connecting the first and last point of the segment, as well as their difference in height, and the mean velocity and acceleration.
%
These features were selected with a cross-validation procedure over a wider set of features. Specifically, during the selection process we considered the following features: the number of points in the segment, the slope of the line connecting the first and last point of the segment, as well as their difference in height, velocity and acceleration, and the minimum, the mean and the maximum velocity and acceleration.
%
We evaluated each feature combination by predicting the controller initial parameters on the qualifier track and then by computing the root-mean-square error (RMSE) of the predicted parameters with respect to the optimal parameters in the training data.
%
Finally, we selected the feature combination that minimized the RMSE.

\subsection{Implementation Choices} \label{subsec:implementation_choices}

\rebuttal{We use the MPC formulation of Falanga~\cite{Falanga2018}, without perception constraints, and the time-optimal planner described by Foehn~\cite{Foehn2020}.
%
We use the AirSim SimpleFlight quadrotor configuration. The quadrotor weights $1.0$ kg and can generate thrust to weight ratio up to $4.179$.
%
We choose the MPC control frequency to be $200$ Hz with horizon step $0.05$.
%
Rather than optimize over the entire optimization landscape, we fix some parameters of the controller to obtain a reduced, but representative, subspace.
%
In particular, we tune the MPC state costs (Q\_pos\_xy, Q\_pos\_z, Q\_attitude, Q\_velocity) and the horizon length, while we fix the MPC input costs (R\_thrust, R\_pitchroll, R\_yaw) to $1.0$, which we experimentally saw to be not very important to performance.
%
Moreover, we bound the inputs to match the limits of the simulator, by fixing the maximum pitch-roll to $10.0$ rad/s, the maximum yaw to $3.0$ rad/s and the maximum thrust to $20.0$ N.
%
The same drone specifics are also used by the time-optimal planner.

We use a Gaussian distribution as proposal function for Metropolis-Hastings algorithm. The distribution is centered on the last set of parameters accepted and has variance $5$, which we empirically found to be effective for our task.
%
At each iteration, the M-H algorithm proposes a new set of parameters by sampling them from the Gaussian distribution.
%
When updating the parameters of a segment, the variance of the preceding segments is reduced by $25\%$.
%
This maintains global optimality but makes the controller close to the previous solution in the preceding segments.
%
We use $e^{-2\sqrt{t}}$, where $t$ is the lap time with added penalty for missed waypoints, as cost function for the M-H algorithm.
}

% \begin{figure*}
%     \centering
%     \setlength{\tabcolsep}{0pt}
%     \begin{tabular}{ccc}
%     \resizebox{0.33\linewidth}{!}{\input{images/tickzfiles/mean}} &
%     \resizebox{0.33\linewidth}{!}{\input{images/tickzfiles/max}} &
%     \resizebox{0.33\linewidth}{!}{\input{images/tickzfiles/error}} \\
%       (a) &
%       (b) &
%       (c) \\
%     \end{tabular}
%     \caption{Results in the real world. After tuning the parameters in simulation, we evaluate the best configuration found by AutoTune on a physical platform. We compare the performance with the controller default parameters. We perform three runs and report the statistics of the mean (a) and max (b) tracking error. We also report the error as a function of time (c) for the best run of our and the default setting. AutoTune consistently improves performance while decreasing the variance between runs.}
%     \label{fig:auto_rw}
% \end{figure*}

\subsection{Choosing Trajectory Segmentation Conditions} \label{app:choosing_traj_segment}

\rebuttal{
Trajectory segmentation is fundamental for successfully tracking high-speed maneuvers. 
%
We split the trajectory into multiple segments according to the height gradient of the reference.
%
Specifically, we assign each point to the class \emph{flat}, \emph{ascent}, or \emph{descent} if the difference in height $g_z = z[k] - z[k+1]$ with its successor is $|g_z|<1m$.
%
The resulting segments are then clustered such that the minimum segment duration is $2$ seconds.
%
Eventually, all the descent and ascent segments with a slope higher than \SI{45}{\degree} are recursively split into two equal parts, where the first is assigned to the class \emph{steep} and the second remains assigned to the original class.

Since the segmentation conditions are crucial to the correct functioning of the proposed algorithm, we study its effects on the tracking performance.
%
Table~\ref{tab:choosing_traj_segment} reports the trajectory completion performance of the proposed algorithm on the Qualifier track. 
%
Each entry of the table is illustrated in Fig.~\ref{fig:choosing_traj_segment}.
%
The reported tracking performance is the best trajectory completion found by the proposed algorithm after $100$ iterations.

The results demonstrate the importance of choosing the right segmentation conditions.
%
By employing high thresholds on height difference and/or minimum duration, the trajectory segmentation method generates only one global segment, thus not allowing different controller behaviors along the track.
%
On the other hand, if the chosen thresholds are too little, then the proposed algorithm cannot find a suitable solution in the limited number of iterations.
%
Therefore, in future work we aim to build a parameter-free automatic segmentation procedure with change-point detection techniques generally used for time series \cite{aminikhanghahi2017KIS}.
}

\newpage

\begin{table}[t]
    \centering
    \begin{tabular}{c c c}
        \toprule
        Height Difference [m] & Min Duration [s] & Trajectory Completion [\%]\\
        \midrule
        1 & 2 & 100\\
        10 & 2 & 100\\
        20 & 2 & 65\\
        30 & 2 & 65\\
        1 & 1 & 60\\
        1 & 5 & 65\\
        \bottomrule
    \end{tabular}
    \caption{Effects of the trajectory segmentation conditions on the tracking performance. The track considered is Qualifier and the metric is the trajectory completion. We assign each point to the class \emph{flat}, \emph{ascent}, or \emph{descent} if the difference in height $g_z = z[k] - z[k+1]$ with its successor is $|g_z|<$\emph{Height Difference}. The resulting segments are then clustered such that the minimum segment duration is \emph{Min Duration} seconds.}
    \label{tab:choosing_traj_segment}
    \vspace{-3ex}
\end{table}

\begin{center}
\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h1d2.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h1d2_seg.png}
\captionof*{figure}{Height Difference $1m$, Min Duration $2s$.}

\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h10d2.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h10d2_seg.png}
\captionof*{figure}{Height Difference $10m$, Min Duration $2s$.}

\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h20d2.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h20d2_seg.png}
\captionof*{figure}{Height Difference $20m$, Min Duration $2s$.}

\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h30d2.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h30d2_seg.png}
\captionof*{figure}{Height Difference $30m$, Min Duration $2s$.}

\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h1d1.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h1d1_seg.png}
\captionof*{figure}{Height Difference $1m$, Min Duration $1s$.}

\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h1d5.eps}
\includegraphics[width=0.49\linewidth]{images/segmentation_conditions/h1d5_seg.png}
\captionof{figure}{Height Difference $1m$, Min Duration $5s$.}
\label{fig:choosing_traj_segment}
\end{center}

\clearpage

\subsection{Controller Stability} \label{app:controller_stability}

\rebuttal{
To increase the stability of the controller between segments, we perform nonlinear MPC optimization with a real-time iteration (RTI) scheme \cite{diehl2009controlstab}. The fact that only a single optimization iteration is done for each timestamp allows a smooth transition of the commanded actions while switching segments. A qualitative analysis is illustrated by Figure~\ref{fig:appendix_control_stab}. The controller's outputs remain smooth over time during switching for any pair of segments.
}

\begin{center}
\includegraphics[width=\linewidth]{images/controller_stability/segment_0.png}
\includegraphics[width=\linewidth]{images/controller_stability/segment_1.png}
\includegraphics[width=\linewidth]{images/controller_stability/segment_2.png}
\captionof{figure}{Effects of parameter change on the stability of the controller on the Drop track. The controller's outputs remain smooth over time during switching for any pair of segments.}
\label{fig:appendix_control_stab}
\end{center}

==> sections/buffer.tex <==




%\begin{itemize}
    %\item The optimization problem of tracking high-speed trajectories. 
    %\item Main difficulty for the controllers is the imperfect model, the Disregard of noise and additional effects difficult to model, and the short horizon.
    %\item There are two available classes of controller: LQR and MPC. We prefer MPC since it's reciding horizon optimization has been proven to be better to cope against disturbances. (book)
    %\item Similarly to previous work, we leave the model unchanged but tune the parameters to maximize performance.
    %\item We find those parameters with M-H sampling.
    %\item To reduce the number of iterations, we initialize the sampling on a low-quality controller, trained with demonstration from different maneuvers.
    %\item Motivated by the observation that different controller behaviors are required in differet part of the trajectory, we propose a strategy to divide the trajectory into parts with different controller. Parameters are different but still optimized jointly.
%\end{itemize}


\section{The Optimization Problem} \label{sec:optimization_problem}

In this section, we formulate the optimization problem. First, the problem is formulated for the general class of controllers. Then, model predictive controllers are presented and the specific optimization problem for these controllers is formulated.

\subsection{Problem Formulation} \label{subsec:problem_statement}

Formally, we are seeking a finite-horizon controller $\pi$, which minimizes the cost over the entire trajectory. Therefore, the objective can be formulated as follows:
\begin{equation} \label{eq:problem_formulation}
    \min_\pi J(\pi) =
    \mathbb{E}_{\rho(\pi)}
    \left[
    \sum_{k=0}^{T} \mathcal{C}(\mbox{\boldmath$\tau$}_r[k], \textbf{s}[k])
    \right],
\end{equation}
where $\mathcal{C}$ is a quadratic cost depending on a reference trajectory $\mbox{\boldmath$\tau$}_r[k]$ and the quadrotor state $\textbf{s}[k]$, and $\rho(\pi)$ is the distribution of possible trajectories induced by the controller $\pi$.

We define the quadrotor state $\textbf{s}[k] = [\textbf{p}, \textbf{q}, \textbf{v}, \mbox{\boldmath$\omega$}]$ as the platform position $\textbf{p}$, its orientation quaternion $\textbf{q}$, and their derivatives. We further define the reference trajectory $\mbox{\boldmath$\tau$}_r[k]$ as a time sequence of reference states which describe the desired trajectory. We formulate the cost $\mathcal{C}$ as
\begin{equation} \label{eq:problem_formulation_general}
    \mathcal{C}(\mbox{\boldmath$\tau$}_r[k], \textbf{s}[k]) =
    \textbf{x}[k]^\top \mathcal{L} \textbf{x}[k],
\end{equation}
where $x[k] = \mbox{\boldmath$\tau$}_r[k] - \textbf{s}[k]$ denotes the difference between the state of the platform and the corresponding reference at time $k$, and $\mathcal{L}$ is a positive-semidefinite cost matrix.

The cost matrix $\mathcal{L}$ is specified by the controller used. Particularly, in this work we concentrate on the class of finite-horizon controllers $\pi$ represented by model predictive controllers.

\subsection{MPC Tuning Problem} \label{subsec:mpc_tuning_problem}

The objective function defined by Eq. \ref{eq:problem_formulation} can be formulated for the class of model predictive controllers as follows:
\begin{equation} \label{eq:problem_formulation_mpc}
    \min_\pi J(\pi) =
    \mathbb{E}_{\rho(\pi)}
    \left[
    \sum_{k=t_0}^{t_h} \textbf{x}[k]^\top \mbox{\boldmath$Q$} \textbf{x}[k] +
    \textbf{u}[k]^\top \mbox{\boldmath$R$} \textbf{u}[k]
    \right],
\end{equation}
where $\mbox{\boldmath$Q$}$ and $\mbox{\boldmath$R$}$ are, resp., the state and input cost matrices, and $h$ is the horizon length. The cost defined by Eq. \ref{eq:problem_formulation_mpc} captures a trade-off between control performance (keeping $\textbf{x}[k]$ small) and control effort (keeping $\textbf{u}[k]$ small).

\subsection{Optimization Landscape} \label{subsec:optimization_landscape}

The optimization landscape is the extent of the domain from which samples can be drawn. For the class of model predictive controllers, the optimization landscape is a $16$-dimensional space: $10$ dimensions are taken from the state cost matrix (position, orientation and velocity), $4$ dimensions are taken from the input cost matrix (yaw, pitch, roll and thrust), and $2$ dimensions are taken from the horizon size (length and step).

The optimization landscape complexity depends on the aggressiveness of the considered trajectory. The faster the trajectory, the more complex the optimization landscape becomes. Examples of optimization landscapes are shown in Fig. \ref{fig:simple_landscape} and Fig. \ref{fig:complex_landscape}. In both examples, an MPC controller is being used for tracking a trajectory. The controller has already being tuned and it is capable of fully tracking the relative trajectory. However, in order to study the optimization landscape, two parameters of the controller are being tuned (x-y plane). For any combination of these two parameters, the trajectory completion percentage is shown (z axis). The trajectory shown in Fig. \ref{fig:simple_landscape} is a minimum-snap trajectory. This class of trajectories minimize the controller tracking effort. Therefore, tuning the controller for flying these trajectories is trivial. The trajectory shown in Fig. \ref{fig:complex_landscape} is a time-optimal trajectory. Flying these trajectories is a challenging task, since at every point of the trajectory the quadrotor is pushed to its actuators physical limits. As a consequence, the generated optimization landscape is complex and uneven.

% \begin{figure*}[h]
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \vspace{-3pt}
%         \includegraphics[width=\textwidth,trim={0 0 0 25},clip]{images/landscape_easy_3d.jpeg}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \vspace{-3pt}
%         \includegraphics[width=\textwidth,trim={0 0 0 25},clip]{images/landscape_easy_2d.png}
%     \end{subfigure}
%     \vspace{-3pt}
%     \caption{Example of optimization landscape produced by tuning a model predictive controller for flying a minimum-snap trajectory. Two parameters of the MPC controller are tuned, namely \textit{Q\_velocity} and \textit{Q\_pos\_xy}. The z axis is defined by the trajectory completion percentage. The generated optimization landscape is smooth and flat.}
%     \label{fig:simple_landscape}
% \end{figure*}
% \begin{figure*}[h]
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \vspace{-3pt}
%         \includegraphics[width=\textwidth,trim={0 0 0 25},clip]{images/landscape_hard_3d.jpeg}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \vspace{-3pt}
%         \includegraphics[width=\textwidth,trim={0 0 0 25},clip]{images/landscape_hard_2d.png}
%     \end{subfigure}
%     \vspace{-3pt}
%     \caption{Example of optimization landscape produced by tuning a model predictive controller for flying a time-optimal trajectory. Two parameters of the MPC controller are tuned, namely \textit{Q\_velocity} and \textit{Q\_pos\_z}. The z axis is defined by the trajectory completion percentage. The optimization landscape is complex and full of local minima. By changing slightly one of the two parameters, the controller performances change significantly.}
%     \label{fig:complex_landscape}
% \end{figure*}

% \clearpage



%%%%%%%%%%%%%%%%%%%% METHOD %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we introduce AutoTune as the optimizer to address the optimization problem (\ref{eq:problem_formulation_mpc}). The key components of AutoTune are explained in Subsec. \ref{subsec:metropolis_hastings} to \ref{subsec:regressors}, while the resulting framework is summarized in Subsec. \ref{subsec:autotune}.

When flying a trajectory, tuning the controller with a set of global parameters may be good enough to allow the quadrotor to successfully track the entire trajectory. However, complex trajectories require different controller behaviors along the track, and global parameters limit the controller to only a particular behavior. For example, consider the complex trajectory illustrated in Fig. \ref{fig:traj_segmentation}. When tracking the purple segment, which lies on the horizontal plane (i.e., the z position of the points in the segment remains constant within a bound), we want the controller to significantly minimize the tracking error of the x-y position of the platform with respect to the reference trajectory. On the other hand, when tracking the green segment, which requires a drop in altitude, we want the controller to significantly minimize the tracking error of the z position of the platform with respect to the reference trajectory.

 \subsection{maybe Summary}
% Write a summary of everything if there is space.


% The prior over the parameters is predicted by using a set of Gradient Boosting regressors trained over previously seen trajectories. Each one of these trajectories have been segmented and a set of parameters have been found for each segment. The set of regressors includes a different regressor for each type of segment (i.e., flat, ascent, descent, drop), so that in total four regressors are used. Each regressor is trained only on segments of the corresponding type.

% During the training phase, the loss function used is Least Squares Regression, the criterion is Mean Squared Error, and the learning rate is equal to $0.1$.

% From each segment, we extract the following features: the number of trajectory points, the mean slope (computed as $s_i = (y_{i+10} - y_{i}) / (x_{i+10} - x_{i})$), and the change in position z, velocity and acceleration.




% The Metropolis-Hastings (M-H) algorithm is a versatile, efficient, and powerful Markov chain Monte Carlo (MCMC) method used to simulate multivariate probability distributions. The algorithm was first developed by Metropolis \cite{Metropolis1953}, and subsequently generalized by Hastings \cite{hastings70}.

% The general schema of the M-H algorithm is summarized in Alg. \ref{alg:metropolis_hastings}. At every iteration, the algorithm picks a candidate for the next sample value based on the current sample value (line $3$). Then, with some probability, the candidate is either accepted (in which case the candidate value is used in the next iteration - line $7$) or rejected (in which case the candidate value is discarded, and current value is reused in the next iteration - line $8$). The probability of acceptance $\alpha$ is determined by comparing the values of the proposal function $f(\textbf{x})$ of the current and candidate sample values with respect to the target distribution $P(\textbf{x})$ (line $5$).

% The M-H algorithm proceeds by randomly attempting to move about the sample space, sometimes accepting the moves and sometimes remaining in place. Note that the acceptance ratio $\alpha$ indicates how probable the new proposed sample is with respect to the current sample, according to the target distribution $P(\textbf{x})$. If we attempt to move to a point that is more probable than the existing point (i.e., a point in a higher-density region of $P(\textbf{x})$), we will always accept the move. However, if we attempt to move to a less probable point, we will sometimes reject the move, and the more the relative drop in probability, the more likely we are to reject the new point. Thus, we will tend to stay in (and return large numbers of samples from) high-density regions of $P(\textbf{x})$, while only occasionally visiting low-density regions. Intuitively, this is why this algorithm works and returns samples that follow the target distribution $P(\textbf{x})$.

% In the context of automatic controller tuning, the target probability distribution $P(\textbf{x})$ is the optimization landscape generated by the controller parameters. The proposal function $f(\textbf{x})$ is usually a multivariate Gaussian distribution. The Gaussian distribution is chosen over other functions for two main reasons: it is symmetric (i.e., $f(\textbf{x} | \textbf{y}) = f(\textbf{y} | \textbf{x})$) and it is specified by only two parameters, the mean and the variance. In this work, the mean is set equal to the last set of parameters accepted, while the variance is an hyper-parameter.

% Figure \ref{fig:metropolis_example} shows the basic steps of the Metropolis-Hastings algorithm.

% \begin{figure}[b]
%     \centering
%     \includegraphics[width=\linewidth]{images/metropolis_algorithm.png}
%     \caption{General schema of the Metropolis-Hastings algorithm.}
%     \label{fig:metropolis_hastings}
% \end{figure}

% \begin{algorithm}[t]
% \caption{Metropolis-Hastings Sampling} \label{alg:metropolis_hastings}
% \KwIn{proposal function $f$, number of iterations $N$, initial parameters $\textbf{q}_{0}$.}
% \KwOut{best-performing set of parameters $\textbf{q}_{best}$.}
% \BlankLine
% \emph{$c_{0} \leftarrow$ evaluate $\textbf{q}_{0}$}\;
% \For{$i \leftarrow 0$ \KwTo $N$}{
% 	\emph{$\textbf{q}' \leftarrow$ propose new parameters from $f(\textbf{q}' | \textbf{q}_{i})$}\;
% 	\emph{$c' \leftarrow$ evaluate $\textbf{q}'$}\;
% 	\emph{$\alpha \leftarrow$ compute the acceptance ratio $c' / c_{i}$}\;
%     \emph{$u \leftarrow$ generate a random number from $[0, 1]$}\;
%     \emph{if $u \leq \alpha$: accept $\textbf{q}'$ and set $\textbf{q}_{i+1}=\textbf{q}'$}\;
%     \emph{if $u > \alpha$: reject $\textbf{q}'$ and set $\textbf{q}_{i+1}=\textbf{q}_{t}$}\;
% }
% \end{algorithm}

% \begin{figure}[b]
%     \centering
%     \includegraphics[width=\linewidth]{images/metropolis_example_horizontal.png}
%     \caption{Illustration of the basic steps of the Metropolis-Hastings algorithm. The light grey shapes depict the target distribution $P(\textbf{x})$. Circles depict parameter combinations within the algorithm. The M-H algorithm proposes a new value conditional on the last one accepted, and accepts (green) or rejects (red) according to the acceptance ratio.}
%     \label{fig:metropolis_example}
% \end{figure}

% \begin{figure}[b]
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/drop_example.png}
%     \caption{Example of drop segment. Drop segments are descent segments with initial angle $\leq 45 ^{\circ}$. The initial angle is calculated with respect to the controller horizon length.}
%     \label{fig:drop_example}
% \end{figure}

% \subsection{The proposed algorithm} \label{subsec:autotune}

% The proposed method for automatic controller tuning is obtained by combining the Metropolis-Hastings algorithm from Sec. \ref{subsec:metropolis_hastings} with the segmentation technique and the set of predictors presented, resp., in Sec. \ref{subsec:segmentation} and Sec. \ref{subsec:regressors}. The automatic controller tuning method is summarized in Alg. \ref{alg:autotune} and illustrated in Fig. \ref{fig:autotune}.

% At every iteration, the algorithm proposes a new controller (line $5$), which is then tested in an experiment to obtain a new cost evaluation (line $6$). By comparing this cost with the evaluation of the last set of parameters accepted, the algorithm accepts or rejects the new controller (lines $7-10$). Through this iterative procedure, the algorithm explores relevant regions of the optimization landscape and eventually yield a set of parameters that allow the quadrotor to successfully track the entire trajectory (line $11$).

% \newpage

% \begin{algorithm}[t]
% \caption{AutoTune Algorithm} \label{alg:autotune}
% \KwIn{proposal function $f$, number of iterations $N$, trajectory $\tau$, set of regressors $R$, stopping condition.}
% \KwOut{best-performing set of parameters $P_{best}$.}
% \BlankLine
% \emph{$S \leftarrow$ split $\tau$ into set of segments}\;
% \emph{$P_0 \leftarrow$ predict parameters $\forall$ segment in $S$ using $R$}\;
% \emph{$c_{0} \leftarrow$ evaluate $P_0$}\;
% \For{$i \leftarrow 0$ \KwTo $N$}{
% 	\emph{$P' \leftarrow$ propose new parameters from $f(P' | P_{i})$}\;
% 	\emph{$c' \leftarrow$ evaluate $P'$}\;
% 	\emph{$\alpha \leftarrow$ compute the acceptance ratio $c' / c_{i}$}\;
%     \emph{$u \leftarrow$ generate a random number from $[0, 1]$}\;
%     \emph{if $u \leq \alpha$: accept $P'$ and set $P_{i+1}=P'$}\;
%     \emph{if $u > \alpha$: reject $P'$ and set $P_{i+1}=P_{t}$}\;
%     \emph{if $stopping\_condition$: return $P_{best}$}\;
% }
% \end{algorithm}



% % simulators
% We validate our approach by tuning controllers for high-speed flight on two different simulators: Microsoft AirSim \cite{madaan2020airsim}, and Flightmare \cite{yunlong2020flightmare}.

% % tracks
% We learn the controllers for flying time-optimal trajectories generated for a set of simulated drone-racing tracks (see Appendix \ref{app:tracks} for the illustration of the considered tracks).
% We learn the controllers for a set of simulated drone-racing tracks. The tracks and relative generated time-optimal trajectories are illustrated in Appendix \ref{app:tracks}.

% % metric
% We define the trajectory completion metric to compare different approaches. The metric is expressed in percentage. We measure the trajectory completion based on the number of gates the platform has passed successfully while tracking the trajectory. 

% % implementation
% We consider the class of model predictive controllers with a similar formulation to Falanga \cite{Falanga2018}.
% The time-optimal planner is the one described by Foehn \cite{Foehn2020}.

\subsubsection{Trajectory Completion Metric} \label{subsubsec:metric}

%We define the trajectory completion metric to compare different approaches.
A trajectory planner requires as input a set of waypoints.
%
We use these waypoints to define the trajectory completion metric to compare different approaches.
%
Specifically, we define the metric as the percentage of waypoints successfully passed while tracking the reference trajectory.
%
A waypoint is considered passed when it is crossed by the platform at an Euclidean distance less than $1.2$ meters.

Fig \ref{fig:metric} illustrates multiple trajectories (grey) flew by the platform while learning the controller for successfully tracking the reference trajectory (blue). 

The reference trajectory is aggressive, reaching a top speed of $53 m/s$ ($190 km/h$). 
The aggressiveness of the trajectory makes learning the controller a very difficult task.

% implementation choices

%%%%%%%%%%%%%%%%%%% EXPERIMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The results demonstrate that the Bayesian optimizer performances depend strongly by the kernel choice. In fact, if one uses a simple kernel (e.g., Rational Quadratic, Periodic), then the random search algorithm returns better performances.
% Bayesian optimization performs poorly since it does not have sufficient information to determine the shape of the optimization landscape.
% The results show that the gap between AutoTune and the other optimization methods widens for more complex and aggressive trajectories, to the point that the proposed approach outperforms the existing algorithms of up to $90\%$.
% As a consequence, AutoTune improves trajectory tracking better than ever before, allowing to track trajectories which previously would have been impractical.


% \begin{figure*}[t]
%     \centering
%     % \caption*{Results}
%     % \vspace{1em}
%     \begin{tabular}{c c c c c}
%         \toprule
%         Method & Soccer\_Field\_Easy & Soccer\_Field\_Easy & Qualifier\_Tier\_1 & Final\_Tier\_1\\
%         & $20$ m/s & $34$ m/s & $20$ m/s & $22$ m/s\\
%         \midrule
%         \textbf{AutoTune} & \textbf{100} & \textbf{100} & \textbf{100} & \textbf{100}\\
%         Random Search & 100 & 65 & 50 & 10\\
%         BO (Mat, EI) & 100 & 80 & 75 & 40\\
%         % BO (Mat, PI) & 100 & 80 & 65 & 40\\
%         BO (LocalPer, EI) & 100 & 65 & 60 & 40\\
%         % BO (LocalPer, PI) & 100 & 50 & 60 & 40\\
%         BO (RQ, EI) & 100 & 60 & 60 & 30\\
%         BO (SQ, EI) & 100 & 60 & 60 & 30\\
%         % BO (RQ, PI) & 100 & 60 & 50 & 30\\
%         % BO (SQ, PI) & 100 & 60 & 50 & 25\\
%         % BO (Per, PI) & 100 & 50 & 50 & 25\\
%         BO (Per, EI) & 100 & 50 & 50 & 25\\
%         \bottomrule
%     \end{tabular}
%     \vspace{1em}
%     \caption{Comparison of AutoTune against different optimization methods in terms of the best trajectory completion percentage over $100$ iterations. Random search and Bayesian optimization perform very poorly as the aggressiveness and the complexity of the trajectory increase. On the contrary, our approach provides a controller that allows the quadrotor to successfully track all the trajectories considered.}
%     \label{tab:optimization_results}
% \end{figure*}

%
% \begin{align} \label{eq:problem_formulation}
%     \min_\pi J(\pi) &=
%     \mathbb{E}_{\rho(\pi)}
%     \left[
%     \sum_{k=0}^{T} (\mbox{\boldmath$\tau$}_r[k] -\textbf{s}[k])^T(\mbox{\boldmath$\tau$}_r[k] -\textbf{s}[k])
%     \right],
% \end{align}
% %
% Given the series of waypoints that the quadrotor is supposed to hit, we use the minimum-time planner of Foehn et al.~\cite{Foehn2020} to compute a reference trajectory $\mbox{\boldmath$\tau$}_r$ passing through all waypoints and respecting the system's actuation and dynamics constraints.
% %
% Flying, or equivalently tracking, this trajectory entails finding a controller $\pi$ that minimizes the quadratic tracking error over the entire trajectory length $T$:

% where $\mbox{\boldmath$\tau$}_r[k]$ is the reference trajectory, $\textbf{s}[k]$ is the quadrotor's state, and $\rho(\pi)$ is the distribution of possible trajectories induced by the controller $\pi$.
% %
% We define the quadrotor state $\textbf{s}[k] = [\textbf{p}, \textbf{q}, \textbf{v}, \mbox{\boldmath$\omega$}]$ as the platform position $\textbf{p}$, its orientation quaternion $\textbf{q}$, and their derivatives. We further define the reference trajectory $\mbox{\boldmath$\tau$}_r[k]$ as a time sequence of reference states that describe the desired trajectory.

A possible choice for the metric $m(w)$ is the tracking error, \emph{i.e.} $m(w) = J(\pi(w))$.

